Positivity of vector bundles and Hodge theory

It is well known that positivity properties of the curvature of a vector bundle have implications on the algebro-geometric properties of the bundle, such as numerical positivity, vanishing of higher cohomology leading to existence of global sections etc. It is also well known that bundles arising in Hodge theory tend to have positivity properties. From these considerations several issues arise: (i) In general for bundles that are semi-positive but not strictly positive; what further natural conditions lead to the existence of sections of its symmetric powers? (ii) In Hodge theory the Hodge metrics generally have singularities; what can be said about these and their curvatures, Chern forms etc.? (iii) What are some algebro-geometric applications of positivity of Hodge bundles? The purpose of these partly expository notes is fourfold. One is to summarize some of the general measures and types of positivity that have arisen in the literature. A second is to introduce and give some applications of norm positivity. This is a concept that implies the di_erent notions of metric semi-positivity that are present in many of the standard examples and one that has an algebro-geometric interpretation in these examples. A third purpose is to discuss and compare some of the types of metric singularities that arise in algebraic geometry and in Hodge theory. Finally we shall present some applications of the theory from both the classical and recent literature.

==> PositivityVBHT(100918)/pgmacs.tex <==
 
   
 \usepackage{graphicx}
%\usepackage[mathx]{mathabx}  %%%needed to allow\widecheck
 \usepackage{epstopdf}
     \usepackage{amssymb}
  \usepackage{color} 
 \usepackage{amsthm,graphpap}
   \newcommand \vfe{\vfill\eject}
   \newcommand\zxi{\zeta}
 \newcommand\CR{{\mathrm{CR}}}
 \newcommand\MHS{{\mathrm{MHS}}}
 \newcommand\rt{{\mathrm{rt}}}
 \newcommand\s{{\mathrm{s}}}
 \newcommand\KU{{\rm KU}}
   \newcommand\cu{\check U}
 \newcommand\qc{quaternionic case}
 \newcommand\xr[1]{\xrightarrow{#1}}
 \newcommand\ull{\mathfrak{l}_\vp}
 \newcommand\tull{\tilde{\mathfrak{l}}_\vp}
 \newcommand\oll{\overline{\mathfrak{l}}}
  \newcommand\vol{\mathop{\rm vol}}
    \newcommand\Id{\mathop{\rm Id}\nolimits}
    \newcommand\ctn{\mathop{\rm ctn}}
    \newcommand\nilp{{\mathrm{nilp}}}
 \let\subest\subset
 \newcommand\vspf{\vspace*{-4pt}}
 \newcommand\vspt{\vspace*{-2pt}}
 \newcommand\lrar{\relbar\hskip-4pt\relbar\hskip-4pt\relbar\hskip-4pt\relbar\hskip-4pt\rightarrow}
 \newcommand\hired[1]{{\color{red} #1}}

\long\def\symbolfootnote[#1]#2{\begingroup%
\def\thefootnote{\fnsymbol{footnote}}\footnote[#1]{#2}\endgroup} 
\newcommand\rhoc{{\rho_c}}

 \newcommand\EC[1]{\marginpar{\tiny #1}}
 
\newcommand\CD{\check{D}}
 
 \newcommand\rmt{{\mathrm{rt}}}
 \newcommand\rmwt{{\mathrm{wt}}}
 
 \newcommand\tdots{\begin{matrix}\cdot\\[-7pt] \cdot\end{matrix}}
 \newcommand\rId{\mathop{\rm Id}\nolimits}
    \newcommand\Def{\mathop{\rm Def}\nolimits}
  \newcommand\bcup{{\ds\mathop{\cup}}\limits}
  \newcommand\Proj{\mathop{\rm Proj}\nolimits}
    \newcommand\Ric{\mathop{\rm Ric}\nolimits}
        \newcommand\reg{\mathop{\rm reg}\nolimits}
    \newcommand\NCD{normal crossing divisor}

 
\newcommand\xrin{\xri{\;N\;}}
\newcommand\fbul{F^\bullet}
\newcommand\fbulp{{F'}^{\bullet}}
\newcommand\fbuly{\fbul_{\infty}}
\newcommand\fbulim{\fbul_{\lim}}
\newcommand\tfbul{\wt F^\bullet}
\newcommand\bbul{{\bullet,\bullet}}
\newcommand\Obul{\Omega^\bullet}
\newcommand\ko{{k_0}}
\newcommand\kop{{k'_0}}
\newcommand\bfbul{\mathbf{f}_\bullet}
\newcommand\bsm{ \begin{smallmatrix}}
\newcommand\bspm{ \left(\begin{smallmatrix}}
\newcommand\esm{\end{smallmatrix} }
\newcommand\espm{\end{smallmatrix} \right)}
\newcommand\bbm{\left[\begin{smallmatrix}}
\newcommand\ebm{\end{smallmatrix}\right]}
\newcommand\bcs{\begin{cases}}
\newcommand\ecs{\end{cases}}
\newcommand\wbul{{W_\bullet}}
 \newcommand{\lra}[1]{\left\langle#1\right\rangle}
\newcommand{\lrc}[1]{\left\{ #1\right\}}
\newcommand{\lrb}[1]{\left[ #1\right]}
\newcommand{\lrp}[1]{\left(#1\right)}
 \newcommand\bp[1]{\bigl(#1\bigr)}
  \newcommand\Bp[1]{\Bigl(#1\Bigr)}
  \newcommand\hmu{{\hat\mu}}
  \newcommand\hX{{\hat X}}
  \newcommand\sump{\mathop{\textstyle \sum'}\limits}
 
  \renewcommand\arraystretch{1.25}
 \newcommand\wt[1]{\widetilde{#1}}
  \newcommand\wh[1]{\widehat{#1}}
 \newcommand\bb{\mathfrak{b}}
 \newcommand\BB{\mathfrak{B}}
 \newcommand\ff{\mathfrak{F}}
 \newcommand\vv{\mathfrak{v}}
 \newcommand\A{\mathbb{A}}
 \newcommand\V{\mathbb{V}}
 \newcommand\W{\mathbb{W}}
 \renewcommand\L{\mathbb{L}}
 \newcommand\bth{\boldsymbol{\theta}}
 \newcommand\bsig{\boldsymbol{\sigma}}
 \newcommand\BPHI{\boldsymbol{\Phi}}
 
 \newcommand\pfrac[2]{\frac{\part #1}{\part #2}}
 
 \newcommand\sidecong{\rotatebox{90}{$\cong$}}
 \newcommand\sidebox{\rotatebox{45}{$\square$}}
  \newcommand\sideeq{\rotatebox{90}{$=$}}
    \newcommand\sidein{\rotatebox{90}{$\in$}}
 \newcommand\ssn[1]{\medbreak\noindent {\bf #1}}
 
 \newcommand\fg{\mathfrak{g}}
\newcommand\hh{\mathfrak{h}}
\newcommand\kk{\mathfrak{k}}
\newcommand\fl{\mathfrak{l}}
\newcommand\mm{\mathfrak{m}}
\newcommand\pp{\mathfrak{p}}
\newcommand\qq{\mathfrak{q}}
\newcommand\rr{\mathfrak{r}}
\renewcommand\tt{\mathfrak{t}}
\newcommand\ttt{\tilde{\tt}}
\newcommand\ww{\mathfrak{w}}
\renewcommand\ss{\mathfrak{s}}

\newcommand{\B}{\mathbb{B}}
\newcommand{\C}{{\mathbb{C}}}
\newcommand{\D}{\mathbb{D}}
\newcommand\E{\mathbb{E}}
\newcommand\F{\mathbb{F}}

\newcommand{\G}{\mathbb{G}}
\newcommand\bH{\mathbb{H}}
\newcommand{\h}{{{\rm I}\hspace*{-2.2pt}{\rm h}}}
\newcommand{\subh}{{{\rm I}\hspace*{-1.3pt}{\rm h}}}
\newcommand{\M}{\mathbb{M}}
 \newcommand\N{\mathbb{N}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\Q}{{\mathbb{Q}}}
\newcommand{\X}{\mathbb{X}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\bS}{{\bf S}}
\newcommand{\T}{\mathbb{T}}
\newcommand{\U}{{\mathbb{U}}}
\newcommand{\Z}{\mathbb{Z}}

 \newcommand\up[1]{^{(#1)}}
 
 \newcommand\ritem[1]{\item[{\rm #1}]}

\newcommand{\cA}{\mathscr{A}}
\newcommand{\cB}{{\mathscr{B}}}
 
\newcommand{\cC}{{\mathscr{C}}}
\newcommand{\cD}{{\mathscr{D}}}
\newcommand{\cE}{{\mathscr{E}}}
\newcommand{\cF}{{\mathscr{F}}}
\newcommand{\cG}{\mathfrak{g}} 
\newcommand\cGC{{\cG_\C}}
\newcommand\cGR{{\cG_\R}}
\newcommand\scG{{\mathscr{G}}}
\newcommand{\cH}{{\mathscr{H}}}
\newcommand{\cI}{{\mathscr{I}}}
\newcommand{\cJ}{{\mathscr{J}}}
\newcommand{\cK}{{\mathscr{K}}}
\newcommand{\cL}{{\mathscr{L}}}
\newcommand{\cl}{{\mathscr{I}}}
\newcommand{\cM}{{\mathscr{M}}}
\newcommand{\cN}{{\mathscr{N}}}
\newcommand{\cO}{{\mathscr{O}}}
\newcommand{\co}{{\scriptstyle\mathscr{O}}}
\newcommand{\sco}{{{\scriptscriptstyle\mathscr{O}}}}
\newcommand{\cP}{{\mathscr{P}}}
\newcommand{\cQ}{{\mathscr{Q}}}
\newcommand{\cR}{{\mathscr{R}}}
\newcommand{\cS}{{\mathscr{S}}}
\newcommand{\cT}{{\mathscr{T}}}
\newcommand{\cU}{{\mathscr{U}}}
\newcommand{\calU}{{\mathscr{U}}}
\newcommand\wtcu{\widetilde{\cU}}
\newcommand\wtcx{\widetilde{\cX}}
\newcommand{\cW}{{\mathscr{W}}}
\newcommand{\cX}{{\mathscr{X}}}
\newcommand{\cY}{{\mathscr{Y}}}
\newcommand{\cZ}{{\mathscr{Z}}}
\newcommand\wtcz{\widetilde{\cZ}}
\newcommand\wtcg{\widetilde{\cG}}
\newcommand\wtczs{\wtcz_\sigma}
\newcommand\bpm{\begin{pmatrix}}
\newcommand\epm{\end{pmatrix}}
 \newcommand\suc{S\cU}

\newcommand\sigo{{}^{\sigma^1}}
\newcommand\sigt{{}^{\sigma^2}}
\newcommand\sigu{{}^\sig}
 
 
 \newcommand\ac{automorphic cohomology}
 \newcommand\mtr{Mumford-Tate representation}
\newcommand\mtd{Mumford-Tate domain}
\newcommand\mtds{Mumford-Tate domain structure}
\newcommand\mtg{Mumford-Tate group}
\newcommand\phs{polarized Hodge structure}
\newcommand\mhs{mixed Hodge structure}
\newcommand\mht{mixed Hodge theory}
\newcommand\lmhs{limiting mixed Hodge structure}
\newcommand\pmhs{polarized mixed Hodge structure}

\newcommand\hd{Hodge domain}
\newcommand\hn{Hodge number}
\newcommand\hb{Hodge bundle}
\newcommand\hg{Hodge group}
\newcommand\hr{Hodge representation}
\newcommand\HR{Hodge-Riemann}
\newcommand\nll{Noether-Lefschetz loci}
\newcommand\mt{Mumford-Tate}
\newcommand\hs{Hodge struc\-ture}
\newcommand\lal{Lie algebra}
\newcommand\Lg{Lie group}

\newcommand\Pic{{\mathop{\rm Pic}\nolimits}}
\newcommand\Hilb{{\mathop{\rm Hilb}\nolimits}}
\newcommand\NL{{\mathop{\rm NL}\nolimits}}
\newcommand\DR{{\mathop{\rm DR}\nolimits}}
\renewcommand\mod{\mathop{\rm mod}\nolimits}
\newcommand\Ad{\mathop{\rm Ad}\nolimits}
\newcommand\rspan{\mathop{\rm span}\nolimits}
\newcommand\SO{\mathop{\rm SO}\nolimits}
\newcommand\so{\mathop{\rm so}\nolimits}
\newcommand\SU{\mathop{\rm SU}\nolimits}
\newcommand\rank{\mathop{\rm rank}\nolimits}

\newcommand\Su{\mathop{\rm Su}\nolimits}
\newcommand\su{\mathop{\rm su}\nolimits}
\newcommand\Sp{\mathop{\rm Sp}\nolimits}
\newcommand\rsp{\mathop{\rm sp}\nolimits}
\newcommand\rsl{\mathop{\rm sl}\nolimits}
\newcommand\HS{\mathop{\rm HS}\nolimits}
\newcommand\MT{\mathop{\rm MT}\nolimits}
\newcommand\Lie{\mathop{\rm Lie}\nolimits}
  \newcommand\HC{Harish-Chandra}
  \newcommand{\gl}{{\rm gl}}
  \newcommand\fgl{\mathfrak{g}\mathfrak{l}}
 \newcommand{\Gr}{\mathop{\rm Gr}\nolimits}
   \newcommand\fGr{\mathfrak{G}\mathfrak{r}}
\newcommand{\Hg}{{\rm Hg}}

\newcommand\CV{\check{V}}
\newcommand\ccU{\check{\cU}}
\newcommand\ccI{\check{\cI}}
\newcommand\ChD{\check{D}}

\newcommand\cz{\check{z}}
\newcommand\ccW{\check{\cW}}
\newcommand\CB{\check{\mathbb{B}}}
\newcommand\CP{\check{\mathbb{P}}}
\newcommand\ccH{\check{\mathcal{H}}}
\newcommand\rid{\mathop{\rm id}\nolimits}
 \newcommand\Aut{\mathop{\rm Aut}\nolimits}
\newcommand\End{\mathop{\rm End}\nolimits}
\newcommand\Fix{\mathop{\rm Fix}\nolimits}
\newcommand\SL{\mathop{\rm SL}\nolimits}
\newcommand\GL{\mathop{\rm GL}\nolimits}
 \newcommand\Grass{\mathop{\rm Grass}\nolimits}
\newcommand\HT{\mathop{\rm HT}\nolimits}
\newcommand\rim{\mathop{\rm Im}\nolimits}
\newcommand\rRe{\mathop{\rm Re}\nolimits}
\newcommand\sing{{\mathop{\rm sing}\nolimits}}
\newcommand\Sym{\mathop{\rm Sym}\nolimits}
\newcommand\id{\mathop{\rm id}\nolimits}
\newcommand\prim{{\rm prim}}
\newcommand\Res{\mathop{\rm Res}\nolimits}
\newcommand\diag{\mathop{\rm diag}\nolimits}
 \newcommand{\Alb}{{\rm Alb}}
\newcommand{\codim}{\mathop{\rm codim}\nolimits}
\newcommand{\Dim}{\mathop{\rm Dim}\nolimits}
\newcommand{\Ext}{\mathop{\rm Ext}\nolimits}
\newcommand{\Tr}{\mathop{\rm Tr}\nolimits}
 \newcommand{\Hom}{\mathop{\rm Hom}\nolimits}
\newcommand{\Ker}{\mathop{\rm Ker}\nolimits}
\newcommand\ad{\mathop{\rm ad}\nolimits}
 
 
\newcommand{\Hdg}{{\rm Hg}}
\newcommand{\AJ}{{\rm AJ}}
\newcommand{\CH}{{\rm CH}}


 \renewcommand{\part}{\partial}
\newcommand{\la}{{\lambda}}
\newcommand\ga{{\gamma}}
\newcommand\Ga{{\Gamma}}
\newcommand{\La}{{\Lambda}}
\newcommand{\Om}{{\Omega}}
\newcommand{\om}{{\omega}}
\newcommand\Sig{{\Sigma}}
\newcommand\bom{\overline{\om}}
\newcommand\vp{\varphi}
\newcommand\sig{\sigma}

\newcommand\tvp{{\widetilde\varphi}}
\newcommand\tD{{\widetilde{D}}}
\newcommand\tG{{\widetilde{G}}}
\newcommand\tF{{\widetilde{F}}}
\newcommand\tL{{\widetilde{L}}}
\newcommand\tT{{\widetilde{T}}}
\newcommand\tY{{\widetilde{Y}}}
\newcommand\tPhi{{\widetilde{\Phi}}}
\newcommand\tmu{{\tilde\mu}}
\newcommand\tS{\widetilde{S}}
\newcommand\ts{\tilde s}

 \newcommand\rmod[1]{\;(\mathop{\rm mod}\nolimits #1)}

\newcommand{\nhs}{\hskip-6pt}
\newcommand{\chs}{\hskip-10pt}
\newcommand\vsp{\vskip8pt plus 2 pt minus 2pt\noindent }
\newcommand\qqquad{\qquad\qquad}
\newcommand\bsl{\backslash}
\newcommand\eps{\epsilon}
\newcommand\vare{\varepsilon}

 
\newcommand\dd{\mathfrak{d}}
\newcommand{\nn}{\mathfrak{n}}
\newcommand{\uu}{\mathfrak{u}}
\newcommand\mfs{\mathfrak{s}}
 \renewcommand{\AA}{{\mathfrak{A}}}
 \newcommand\ZZ{\mathfrak{Z}}
\newcommand\cnn{\check{\nn}}
\newcommand\ctt{\check{\tt}}
\newcommand{\lab}{\label}
\newcommand\pref[1]{{\rm (\ref{#1})}}


  \renewcommand\theenumi{\roman{enumi}}
   \newcommand\isep{\parskip-2mm  \itemsep3mm}

\newcommand{\hensp}[1]{\enspace\hbox{#1}\enspace}


\newcommand{\opplus}{\mathop{\oplus}\limits}
\newcommand{\ottimes}{\mathop{\otimes}\limits}

\newcommand\mup{{\mu'}}
\newcommand\pip{{\pi'}}


  \renewcommand\thesection{\arabic{section}}
 

 \renewcommand\thesubsection{\thesection.\arabic{subsection}}
 
\newcounter{demo}[equation]
   \renewcommand{\thedemo}{\thesection.\arabic{equation}}

 \newenvironment{demo}{
 \addtocounter{equation}{1}\refstepcounter{demo} \setcounter{demo}{\value{equation} }
{\smallbreak\noindent (\thesection.\arabic{demo})\enspace   }} 
 
 \newtheoremstyle{mytheo}% name
 {3pt}%      Space above
  {3pt}%      Space below
  {\itshape}%         Body font
  {}%         Indent amount (empty = no indent, \parindent = para indent)
  {\scshape}% Thm head font
  {:}%        Punctuation after thm head
  {.5em}%     Space after thm head: " " = normal interword space;
        %       \newline = linebreak
  {}%         Thm head spec (can be left empty, meaning `normal')

\theoremstyle{mytheo}
\newtheorem*{cor}{Corollary}
\newtheorem{Cor}[equation]{Corollary}
\newtheorem{thm}{Theorem}
\newtheorem{Thm}[equation]{Theorem}
  \newtheorem*{conj}{Conjecture}
  \newtheorem{Conj}[equation]{Conjecture}
\renewcommand\thethm{\Roman{thm}}
\newtheorem{Lem}[equation]{Lemma}
 \newtheorem*{lem}{Lemma}
\newtheorem{thmp}{Theorem}
\newtheorem{claim}[equation]{Claim}
\renewcommand\thethmp{\Roman{thm}$'$}
 \newtheorem*{quest}{Question}
\newtheorem*{propn}{Proposition}
\newtheorem{Prop}[equation]{Proposition}
\newtheorem*{propast}{$(\ast)$\; Proposition}
 \newtheorem*{bhl}{Bruhat's Lemma}
\newtheorem*{thmn}{Theorem}
 \newtheorem{Concls}[equation]{Conclusions}
\newtheoremstyle{note}% name
  {3pt}%      Space above
  {3pt}%      Space below
  {}%         Body font
  {}%         Indent amount (empty = no indent, \parindent = para indent)
  {\bfseries}% Thm head font
  {:}%        Punctuation after thm head
  {.5em}%     Space after thm head: " " = normal interword space;
        %       \newline = linebreak
  {}%         Thm head spec (can be left empty, meaning `normal')
\theoremstyle{note}

\newtheorem{Defin}[equation]{Definition}
\newtheorem*{apps}{Applications}
\newtheorem*{appsmd}{Minimal degeneration}
\newtheorem*{maxdeg}{Maximal degenerations to a closed orbit of the form $G_\R/Q_\R$}
 \newtheorem*{defs}{Definitions}
\newtheorem*{defin}{Definition}
 \newtheorem*{conc}{Conclusion}
\newtheorem*{defis}{Definitions}
 \newtheorem*{exam}{Example}
\newtheorem*{exams}{Examples}
\newtheorem{Exam}[equation]{Example}
\newtheorem{example}{Example}
\newtheorem*{rems}{Remarks}
\newtheorem*{rem}{Remark}
\newtheorem*{anote}{Note}
\newtheorem*{notes}{Notes}
\newtheorem*{Idea}{Idea}
\newtheorem{Rem}[equation]{Remark}
 
\newtheorem*{nota}{Notation}
\theoremstyle{remark}
\newtheorem{step}{Step}

 
\newcommand\simto{\xrightarrow{\sim}}
\newcommand\xri[1]{\xrightarrow{#1}}
\newcommand\bu{\mathbf{u}}
\newcommand\bx{\mathbf{x}}
\newcommand\bt{\mathbf{t}}
\newcommand\bc{\mathbf{c}}
\newcommand\bk{\mathbf{k}}
\newcommand\bB{\mathbf{B}}
\newcommand\bG{\mathbf{G}}
\newcommand\bI{\mathbf{I}}
\newcommand\bw{\mathbf{w}}
\newcommand\bC{\mathbf{C}}
\newcommand\bP{\mathbf{P}}
\newcommand\bQ{\mathbf{Q}}



\newcommand\ol[1]{\overline{#1}}
\newcommand\ola{{\overline{\alpha}}}
\newcommand\olb{{\overline{\beta}}}

\newcommand\ogq{\overline{\Ga}^{\mkern2 mu \Q}}
\newcommand\oV[1]{\overline{V}^{\mkern2mu #1}}
\newcommand\lot{\mathop{\rm LoT}\nolimits}
\def\ribitem#1{\item[{[#1]}]}
 \usepackage[mathscr]{euscript}
\input{xy}
\xyoption{all}
  \renewcommand\thesection{\arabic{section}}
 

 \renewcommand\thesubsection{\thesection.\Alph{subsection}}

%\renewcommand{\theequation}{\thesection.\arabic{equation}} 
